Extrapolated Shock Tracking: Bridging shock-fitting and embedded boundary methods

We propose a novel approach to approximate numerically shock waves. The method combines the unstructured shock-fitting approach developed in the last decade by some of the authors, with ideas coming from embedded boundary techniques. The numerical method obtained allows avoiding the re-meshing phase required by the unstructured fitting method, while guaranteeing accuracy properties very close to those of the fitting approach. This new method has many similarities with front tracking approaches, and paves the way to shock-tracking techniques truly independent on the data and mesh structure used by the flow solver. The approach is tested on several problems showing accuracy properties very close to those of more expensive fitting methods, with a considerable gain in flexibility and generality.

==> log <==
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019/TeX Live for SUSE Linux) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./manuscript.tex
LaTeX2e <2018-12-01>
(/usr/share/texmf/tex/latex/elsevier/elsarticle.cls
Document Class: elsarticle 2009/09/17, 1.2.0: Elsevier Ltd
(/usr/share/texmf/tex/latex/base/article.cls
Document Class: article 2018/09/03 v1.4i Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size12.clo))
(/usr/share/texmf/tex/latex/graphics/graphicx.sty
(/usr/share/texmf/tex/latex/graphics/keyval.sty)
(/usr/share/texmf/tex/latex/graphics/graphics.sty
(/usr/share/texmf/tex/latex/graphics/trig.sty)
(/usr/share/texmf/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texmf/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texmf/tex/latex/psnfss/pifont.sty
(/usr/share/texmf/tex/latex/psnfss/upzd.fd)
(/usr/share/texmf/tex/latex/psnfss/upsy.fd)) (./manuscript.spl)
(/usr/share/texmf/tex/latex/natbib/natbib.sty))
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf/tex/latex/amscls/amsthm.sty)
(/usr/share/texmf/tex/latex/subfig/subfig.sty
(/usr/share/texmf/tex/latex/caption/caption.sty
(/usr/share/texmf/tex/latex/caption/caption3.sty)))
(/usr/share/texmf/tex/latex/graphics/color.sty
(/usr/share/texmf/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf/tex/latex/tools/tabularx.sty
(/usr/share/texmf/tex/latex/tools/array.sty))
(/usr/share/texmf/tex/latex/booktabs/booktabs.sty) (./manuscript.aux

LaTeX Warning: Label `fig:cont' multiply defined.

) (/usr/share/texmf/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texmf/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texmf/tex/latex/oberdiek/grfext.sty
(/usr/share/texmf/tex/generic/oberdiek/kvdefinekeys.sty
(/usr/share/texmf/tex/generic/oberdiek/ltxcmds.sty)))
(/usr/share/texmf/tex/latex/oberdiek/kvoptions.sty
(/usr/share/texmf/tex/generic/oberdiek/kvsetkeys.sty
(/usr/share/texmf/tex/generic/oberdiek/etexcmds.sty
(/usr/share/texmf/tex/generic/oberdiek/ifluatex.sty))))
(/usr/share/texmf/tex/generic/oberdiek/pdftexcmds.sty
(/usr/share/texmf/tex/generic/oberdiek/ifpdf.sty))
(/usr/share/texmf/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd) (./introduction.tex [1{/var/lib/t
exmf/fonts/map/pdftex/updmap/pdftex.map}] [2] [3] [4] [5] [6] [7 <./figure20a-e
ps-converted-to.pdf> <./ss3-f3-eps-converted-to.pdf> <./shk1_TC3_new-eps-conver
ted-to.pdf>] [8]
Underfull \hbox (badness 1132) in paragraph at lines 269--269
[]\OT1/cmr/m/n/10 (a) |The sur-ro-gate bound-ary $[]$ and true


pdfTeX warning: pdflatex (file ./SBM2-eps-converted-to.pdf): PDF inclusion: fou
nd PDF version <1.7>, but at most version <1.5> allowed
[9 <./potato.png> <./SBM2-eps-converted-to.pdf>]
Overfull \hbox (15.344pt too wide) in paragraph at lines 303--304
[]\OT1/cmr/m/n/12 Geometrical cou-pling of the shock-
[10]) (./SSFalgorithm.tex [11]

LaTeX Warning: `h' float specifier changed to `ht'.

[12] [13 <./figure0.pdf> <./figure1.pdf>] [14 <./figure2.pdf>] [15] [16 <./figu
re3.pdf>]
Underfull \hbox (badness 10000) in paragraph at lines 531--532

[17 <./figure4.pdf>]
Underfull \hbox (badness 10000) in paragraph at lines 639--643


Underfull \hbox (badness 10000) in paragraph at lines 644--645

[18]
Underfull \hbox (badness 10000) in paragraph at lines 759--760


Underfull \hbox (badness 10000) in paragraph at lines 761--762

[19 <./figure5.pdf>] [20 <./figure6.pdf>] [21 <./figure7.pdf>]
Overfull \hbox (9.39586pt too wide) in paragraph at lines 1187--1191
[]\OT1/cmr/m/n/12 During the shock dis-place-ment step, the shock-edges may str
etch or shorten,
) (./Q1D.tex [22 <./figure8.pdf>] [23]

pdfTeX warning: pdflatex (file ./conv1D_1-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./conv1D_2-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed
[24 <./conv1D_1-eps-converted-to.pdf>] [25 <./conv1D_2-eps-converted-to.pdf>]

pdfTeX warning: pdflatex (file ./Q1Dsketch-eps-converted-to.pdf): PDF inclusion
: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./mesh_SC-eps-converted-to.pdf): PDF inclusion: 
found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./Q1D_SSF-SC_S-Z3-eps-converted-to.pdf): PDF inc
lusion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./Q1D-shock-eps-converted-to.pdf): PDF inclusion
: found PDF version <1.7>, but at most version <1.5> allowed

Overfull \hbox (2.61108pt too wide) in paragraph at lines 151--155
[][]  [] 
[26 <./Q1Dsketch-eps-converted-to.pdf> <./mesh_SC-eps-converted-to.pdf>]

pdfTeX warning: pdflatex (file ./conv2D-1-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed
[27 <./Q1D_SSF-SC_S-Z3-eps-converted-to.pdf> <./Q1D-shock-eps-converted-to.pdf>
]

pdfTeX warning: pdflatex (file ./conv2D-2_2-eps-converted-to.pdf): PDF inclusio
n: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./conv2D-2-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed

Underfull \hbox (badness 10000) in alignment at lines 211--211
[][][][] 
) (./Computational_cost.tex [28 <./conv2D-1-eps-converted-to.pdf>] [29 <./conv2
D-2_2-eps-converted-to.pdf> <./conv2D-2-eps-converted-to.pdf>]
Overfull \hbox (16.67633pt too wide) in paragraph at lines 5--11
\OT1/cmr/m/n/12 tech-niques to achieve the same discretization-error level in t
he shock-downstream
[30]) (./BluntBody.tex [31]

pdfTeX warning: pdflatex (file ./CCsketch-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC_SSF-SC_P_2-eps-converted-to.pdf): PDF inclu
sion: found PDF version <1.7>, but at most version <1.5> allowed
[32 <./CCsketch-eps-converted-to.pdf>]

pdfTeX warning: pdflatex (file ./shock_layer_SC-SSF-SF-eps-converted-to.pdf): P
DF inclusion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC-fitting1-eps-converted-to.pdf): PDF inclusi
on: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC-fitting2-eps-converted-to.pdf): PDF inclusi
on: found PDF version <1.7>, but at most version <1.5> allowed
) (./HybridComputations.tex
Underfull \hbox (badness 10000) in paragraph at lines 4--6

[33 <./CC_SSF-SC_P_2-eps-converted-to.pdf>]

pdfTeX warning: pdflatex (file ./HYB1sketch-eps-converted-to.pdf): PDF inclusio
n: found PDF version <1.7>, but at most version <1.5> allowed

LaTeX Warning: `!h' float specifier changed to `!ht'.



pdfTeX warning: pdflatex (file ./HYB1_SSF-SC_M-eps-converted-to.pdf): PDF inclu
sion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./HYB1TP_SSF-SC_M-eps-converted-to.pdf): PDF inc
lusion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./HYB1mach-TP_SSF-SC_M-eps-converted-to.pdf): PD
F inclusion: found PDF version <1.7>, but at most version <1.5> allowed

LaTeX Warning: `!h' float specifier changed to `!ht'.

[34 <./shock_layer_SC-SSF-SF-eps-converted-to.pdf>]

pdfTeX warning: pdflatex (file ./HYB-fitting1-eps-converted-to.pdf): PDF inclus
ion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./HYB-fitting2-eps-converted-to.pdf): PDF inclus
ion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./SSIVsketch-eps-converted-to.pdf): PDF inclusio
n: found PDF version <1.7>, but at most version <1.5> allowed
[35 <./CC-fitting1-eps-converted-to.pdf> <./CC-fitting2-eps-converted-to.pdf>]

pdfTeX warning: pdflatex (file ./SSIV_SC-M1-eps-converted-to.pdf): PDF inclusio
n: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./SSIV_SSF-M1-eps-converted-to.pdf): PDF inclusi
on: found PDF version <1.7>, but at most version <1.5> allowed

Overfull \hbox (3.91663pt too wide) in paragraph at lines 90--94
 [][][] 

LaTeX Warning: `!h' float specifier changed to `!ht'.

) (./Conclusion.tex [36 <./HYB1sketch-eps-converted-to.pdf>] [37 <./HYB1_SSF-SC
_M-eps-converted-to.pdf> <./HYB1TP_SSF-SC_M-eps-converted-to.pdf> <./HYB1mach-T
P_SSF-SC_M-eps-converted-to.pdf> <./HYB-fitting1-eps-converted-to.pdf> <./HYB-f
itting2-eps-converted-to.pdf>] [38 <./SSIVsketch-eps-converted-to.pdf>])
(./Appendix.tex [39 <./SSIV_SC-M1-eps-converted-to.pdf> <./SSIV_SSF-M1-eps-conv
erted-to.pdf>] [40 <./figure10.pdf> <./figure9.pdf>]
Overfull \hbox (4.27368pt too wide) in paragraph at lines 117--118
[]\OT1/cmr/m/n/12 The gra-di-ent re-con-struc-tion de-scribed so far ap-plies t
o the two-dimensional
[41 <./figure11.pdf>]

pdfTeX warning: pdflatex (file ./Q1D-iter1-eps-converted-to.pdf): PDF inclusion
: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./Q1D-iter201-eps-converted-to.pdf): PDF inclusi
on: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./Q1D-final-eps-converted-to.pdf): PDF inclusion
: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC-iter1-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC-iter101-eps-converted-to.pdf): PDF inclusio
n: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC-final-eps-converted-to.pdf): PDF inclusion:
 found PDF version <1.7>, but at most version <1.5> allowed

LaTeX Warning: `!h' float specifier changed to `!ht'.



pdfTeX warning: pdflatex (file ./HYB-iter1-eps-converted-to.pdf): PDF inclusion
: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./HYB-iter201-eps-converted-to.pdf): PDF inclusi
on: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./HYB-final-eps-converted-to.pdf): PDF inclusion
: found PDF version <1.7>, but at most version <1.5> allowed

LaTeX Warning: `!h' float specifier changed to `!ht'.



pdfTeX warning: pdflatex (file ./Q1D_shkspeed-eps-converted-to.pdf): PDF inclus
ion: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./CC_shkspeed-eps-converted-to.pdf): PDF inclusi
on: found PDF version <1.7>, but at most version <1.5> allowed


pdfTeX warning: pdflatex (file ./HYB_shkspeed-eps-converted-to.pdf): PDF inclus
ion: found PDF version <1.7>, but at most version <1.5> allowed

LaTeX Warning: `!h' float specifier changed to `!ht'.

) (./manuscript.bbl [42 <./Q1D-iter1-eps-converted-to.pdf> <./Q1D-iter201-eps-c
onverted-to.pdf> <./Q1D-final-eps-converted-to.pdf>] [43 <./CC-iter1-eps-conver
ted-to.pdf> <./CC-iter101-eps-converted-to.pdf> <./CC-final-eps-converted-to.pd
f> <./HYB-iter1-eps-converted-to.pdf> <./HYB-iter201-eps-converted-to.pdf> <./H
YB-final-eps-converted-to.pdf>] [44 <./Q1D_shkspeed-eps-converted-to.pdf> <./CC
_shkspeed-eps-converted-to.pdf> <./HYB_shkspeed-eps-converted-to.pdf>] [45]
[46]
Underfull \hbox (badness 2913) in paragraph at lines 168--176
[]\OT1/cmr/m/n/12 R. Pa-ciorri, A. Bon-figli-oli, Ac-cu-rate de-tec-tion of sho
ck waves

Underfull \hbox (badness 6236) in paragraph at lines 168--176
\OT1/cmr/m/n/12 and shock in-ter-ac-tions in two-dimensional shock-capturing so
-

Underfull \hbox (badness 3954) in paragraph at lines 168--176
\OT1/cmr/m/n/12 lu-tions, Jour-nal of Com-pu-ta-tional Physics 406 (2020) 10919
6.

Overfull \hbox (69.1095pt too wide) in paragraph at lines 168--176
\OT1/cmr/m/n/12 URL \OT1/cmtt/m/n/12 http://www.sciencedirect.com/science/artic
le/pii/S0021999119309015 
[47]
Underfull \hbox (badness 10000) in paragraph at lines 225--227
[]\OT1/cmr/m/n/12 J. Shewchuk, Tri-an-gle mesh gen-er-a-tor, Avail-able at
[48]
Underfull \hbox (badness 10000) in paragraph at lines 251--258
[]\OT1/cmr/m/n/12 F. Alauzet, A. Lo-seille, G. Olivier, Time-accurate multi-

Underfull \hbox (badness 10000) in paragraph at lines 251--258
\OT1/cmr/m/n/12 scale anisotropic mesh adap-ta-tion for un-steady flows in

Underfull \hbox (badness 4779) in paragraph at lines 251--258
\OT1/cmr/m/n/12 cfd, Jour-nal of Com-pu-ta-tional Physics 373 (2018) 28 -- 63.

Overfull \hbox (69.1095pt too wide) in paragraph at lines 251--258
\OT1/cmr/m/n/12 URL \OT1/cmtt/m/n/12 http://www.sciencedirect.com/science/artic
le/pii/S0021999118304212 

Underfull \hbox (badness 10000) in paragraph at lines 265--267
[]\OT1/cmr/m/n/12 J. M^^?uller, De-laundo mesh gen-er-a-tor, Avail-able at
) [49] (./manuscript.aux)

LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information)</usr/share/texmf/fonts/typ
e1/public/amsfonts/cm/cmbx10.pfb></usr/share/texmf/fonts/type1/public/amsfonts/
cm/cmbx12.pfb></usr/share/texmf/fonts/type1/public/amsfonts/cm/cmbx8.pfb></usr/
share/texmf/fonts/type1/public/amsfonts/cm/cmbxti10.pfb></usr/share/texmf/fonts
/type1/public/amsfonts/cm/cmex10.pfb></usr/share/texmf/fonts/type1/public/amsfo
nts/cm/cmmi10.pfb></usr/share/texmf/fonts/type1/public/amsfonts/cm/cmmi12.pfb><
/usr/share/texmf/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/share/texmf/fon
ts/type1/public/amsfonts/cm/cmmi7.pfb></usr/share/texmf/fonts/type1/public/amsf
onts/cm/cmmi8.pfb></usr/share/texmf/fonts/type1/public/amsfonts/cm/cmmib10.pfb>
</usr/share/texmf/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/share/texmf/fo
nts/type1/public/amsfonts/cm/cmr12.pfb></usr/share/texmf/fonts/type1/public/ams
fonts/cm/cmr17.pfb></usr/share/texmf/fonts/type1/public/amsfonts/cm/cmr6.pfb></
usr/share/texmf/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/share/texmf/fonts
/type1/public/amsfonts/cm/cmr8.pfb></usr/share/texmf/fonts/type1/public/amsfont
s/cm/cmsy10.pfb></usr/share/texmf/fonts/type1/public/amsfonts/cm/cmsy6.pfb></us
r/share/texmf/fonts/type1/public/amsfonts/cm/cmsy8.pfb></usr/share/texmf/fonts/
type1/public/amsfonts/cm/cmti10.pfb></usr/share/texmf/fonts/type1/public/amsfon
ts/cm/cmti12.pfb></usr/share/texmf/fonts/type1/public/amsfonts/cm/cmti7.pfb></u
sr/share/texmf/fonts/type1/public/amsfonts/cm/cmtt12.pfb></usr/share/texmf/font
s/type1/public/amsfonts/symbols/msbm10.pfb>
Output written on manuscript.pdf (49 pages, 10140398 bytes).
Transcript written on manuscript.log.

